Fare Zone Assignment on Trees

Designing fare systems for public transportation networks is a challenging task. A popular approach is to partition the network into fare zones (``zoning'') and fix journey prices depending on the number of traversed zones (``pricing''). In this paper, we focus on finding revenue-optimal solutions to the zoning problem for a given subadditive pricing function. We consider tree networks with $n$ vertices, since trees already pose non-trivial algorithmic challenges. Our main results are efficient algorithms that yield a simple $\mathcal{O}(\log n)$-approximation as well as a more involved $\mathcal{O}(\log n/\log \log n)$-approxi\-ma\-tion. We show that rooted instances, in which all demand arises at a single source, can be solved exactly. We further show APX-hardness for general instances on star graphs. For paths, we prove strong NP-hardness and outline a PTAS. Moreover, we show that computing an optimal solution is in FPT or XP for several natural problem parameters.

==> TikzSet.tex <==
\makeatletter
\tikzset{
	circle split part fill/.style  args={#1,#2}{%
		alias=tmp@name,
		postaction={%
			insert path={
				\pgfextra{% 
					\pgfpointdiff{\pgfpointanchor{\pgf@node@name}{center}}%
					{\pgfpointanchor{\pgf@node@name}{east}}%            
					\pgfmathsetmacro\insiderad{\pgf@x}
					%\begin{scope}[on background layer]
					%\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
					%                    (0:180:\insiderad-0.5\pgflinewidth)--cycle;
					%\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
					%                     (180:360:\insiderad-0.5\pgflinewidth)--cycle;  
					\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
					(0:180:\insiderad-\pgflinewidth)--cycle;
					\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
					(180:360:\insiderad-\pgflinewidth)--cycle;  
	}}}},
	rectangle split part fill/.style  args={#1,#2}{%
		alias=tmp@name,
		postaction={%
			insert path={
				\pgfextra{% 
					\pgfpointdiff{\pgfpointanchor{\pgf@node@name}{center}}%
					{\pgfpointanchor{\pgf@node@name}{east}}%            
					\pgfmathsetmacro\insiderad{\pgf@x}
					%\begin{scope}[on background layer]
					%\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
					%                    (0:180:\insiderad-0.5\pgflinewidth)--cycle;
					%\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
					%                     (180:360:\insiderad-0.5\pgflinewidth)--cycle;  
					\fill[#1] (\pgf@node@name.west) -- (\pgf@node@name.north west) -- (\pgf@node@name.north east) -- (\pgf@node@name.east) -- (\pgf@node@name.west);
					\fill[#2] (\pgf@node@name.west) -- (\pgf@node@name.south west) -- (\pgf@node@name.south east) -- (\pgf@node@name.east) -- (\pgf@node@name.west); 
					\draw[thick] (\pgf@node@name.north west) -- (\pgf@node@name.south west) -- (\pgf@node@name.south east) -- (\pgf@node@name.north east) -- (\pgf@node@name.north west) -- (\pgf@node@name.south west); 
	}}}},
}  
\makeatother  
%
%\newlength{\kandinsky} %defines a new length 
%\settowidth{\kandinsky}{\footnotesize Wassily Kandinsky} 
%set new length for the proper parbox width
\makeatletter
\tikzset{
	every node/.style={
		%thick,
		%circle,
		inner sep = 0pt,
		outer sep = 0pt,
		minimum size = .7cm,
		draw,
		%line width=1mm,
	},
	plain/.style={
		draw = none,
		fill = none,
		minimum size = .6cm
	},
	aPartition/.style={
		%fill = graphcolorpeach-orange,
		shape = rectangle,
	},
	bPartition/.style={
		%fill = graphcolorpeach,
		shape = circle
	},
	background/.style={
		opacity=.40,
		fill = gray,       
	},
	cover/.style={
		fill = RWTH_Magenta,
		text = white
	},
%	priceable/.style={
%		fill = RWTH_Magenta,
%		text = white,
%		%very thick,
%	},
%	fixed price/.style={
%		fill = rwthblue,
%		text = white,
%		very thick,
%	},
	CoreCoverA/.style={
		rectangle split part fill={RWTH_Magenta, rwthblue},
		text = white,
	},
	CoreCoverB/.style={
		circle split part fill={RWTH_Magenta, rwthblue},
		text = white,
	},
	CoreComplementA/.style={
		rectangle split part fill={rwthblue_25prcnt, rwthblue},
		text = white,
	},
	CoreComplementB/.style={
		circle split part fill={rwthblue_25prcnt, rwthblue},
		text = white,
	},
%	priceable CoverB/.style={
%		%circle split part fill={RWTH_Magenta, rwthblue},  
%		circle split part fill={RWTH_Magenta, RWTH_Lightblue}, 
%		text = white,
%		thick,	
%	},
%	fixed price CoverA/.style={
%		%circle split part fill={RWTH_Magenta, rwthblue},  
%		rectangle split part fill={rwthblue, RWTH_Lightblue}, 
%		text = white,
%		thick,	
%	},
%	fixed price CoverB/.style={
%		%circle split part fill={RWTH_Magenta, rwthblue},  
%		circle split part fill={rwthblue, RWTH_Lightblue}, 
%		text = white,
%		thick,	
%	},
	blue/.style={
		fill = rwthblue,
		text = white
	},
	light blue/.style={
		fill = rwthblue_25prcnt,
		text = white
	},
	magenta/.style={
		fill = RWTH_Magenta,
		text = white
	},
	complementEdge/.style={
		dashed,
		color = black
	},
	backgroundEdge/.style={
		opacity = .5,
		dashed
	},
	textbox/.style={
		shape = rectangle,
		draw = none,
		minimum height=\textboxHeight,
		inner ysep = 0cm,
		inner xsep = .1cm,
		outer sep = 0cm,
	},
	vertex/.style={
		inner sep = 0cm,
		outer sep = 0cm,
		minimum size=.85cm,
		draw
	}
}
\makeatother 

\newlength{\textboxHeight} %defines a new length 
\setlength{\textboxHeight}{.53cm}
\newlength{\vertSpacing} %defines a new length 
\setlength{\vertSpacing}{.5cm}
\newlength{\fullVertSpacing}
\setlength{\fullVertSpacing}{\vertSpacing}
\addtolength{\fullVertSpacing}{\vertSpacing}
\addtolength{\fullVertSpacing}{\textboxHeight}
